A General Decomposition Method for a Convex Problem Related to Total Variation Minimization

We consider sequential and parallel decomposition methods for a dual problem of a general total variation minimization problem with applications in several image processing tasks, like image inpainting, estimation of optical flow and reconstruction of missing wavelet coefficients. The convergence of these methods to a solution of the global problem is analysed in a Hilbert space setting and a convergence rate is provided. Thereby, these convergence result hold not only for exact local minimization but also if the subproblems are just solved approximately. As a concrete example of an approximate local solution process a surrogate technique is presented and analysed. Further, the obtained convergence rate is compared with related results in the literature and shown to be in agreement with or even improve upon them. Numerical experiments are presented to support the theoretical findings and to show the performance of the proposed decomposition algorithms in image inpainting, optical flow estimation and wavelet inpainting tasks.

==> data1/fd/convergence/denoising/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/\DataPrefix/lambda\endcsname{\pgfmathprintnumber{0.1}}
\expandafter\def\csname Data/\DataPrefix/beta\endcsname{\pgfmathprintnumber{0.0}}
\expandafter\def\csname Data/\DataPrefix/tau\endcsname{\pgfmathprintnumber{0.125}}
\expandafter\def\csname Data/\DataPrefix/maxiters\endcsname{\pgfmathprintnumber{10000}}
\expandafter\def\csname Data/\DataPrefix/ninner\endcsname{\pgfmathprintnumber{100}}
\expandafter\def\csname Data/\DataPrefix/noise_sigma\endcsname{\pgfmathprintnumber{0.1}}
\expandafter\def\csname Data/\DataPrefix/energymin\endcsname{\pgfmathprintnumber{456.60535683028445}}
\expandafter\def\csname Data/\DataPrefix/width\endcsname{\pgfmathprintnumber{48}}
\expandafter\def\csname Data/\DataPrefix/height\endcsname{\pgfmathprintnumber{32}}


==> data1/fd/convergence/denoising/params.tex <==
\providecommand{\Parameter}[1]{
  \csname Parameter/#1\endcsname
}
\expandafter\def\csname Parameter/convergence/denoising/a\endcsname{1}
\expandafter\def\csname Parameter/convergence/denoising/b\endcsname{7}


==> data1/fd/convergence/inpainting/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/\DataPrefix/lambda\endcsname{\pgfmathprintnumber{0.05}}
\expandafter\def\csname Data/\DataPrefix/beta\endcsname{\pgfmathprintnumber{0.001}}
\expandafter\def\csname Data/\DataPrefix/tau\endcsname{\pgfmathprintnumber{0.000125}}
\expandafter\def\csname Data/\DataPrefix/maxiters\endcsname{\pgfmathprintnumber{10000}}
\expandafter\def\csname Data/\DataPrefix/ninner\endcsname{\pgfmathprintnumber{100}}
\expandafter\def\csname Data/\DataPrefix/energymin\endcsname{\pgfmathprintnumber{226.3738646560107}}
\expandafter\def\csname Data/\DataPrefix/width\endcsname{\pgfmathprintnumber{48}}
\expandafter\def\csname Data/\DataPrefix/height\endcsname{\pgfmathprintnumber{32}}


==> data1/fd/convergence/opticalflow/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/\DataPrefix/lambda\endcsname{\pgfmathprintnumber{0.002}}
\expandafter\def\csname Data/\DataPrefix/beta\endcsname{\pgfmathprintnumber{0.001}}
\expandafter\def\csname Data/\DataPrefix/tau\endcsname{\pgfmathprintnumber{0.00012499999999999873}}
\expandafter\def\csname Data/\DataPrefix/maxiters\endcsname{\pgfmathprintnumber{10000}}
\expandafter\def\csname Data/\DataPrefix/ninner\endcsname{\pgfmathprintnumber{100}}
\expandafter\def\csname Data/\DataPrefix/energymin\endcsname{\pgfmathprintnumber{0.06736125560394604}}
\expandafter\def\csname Data/\DataPrefix/width\endcsname{\pgfmathprintnumber{48}}
\expandafter\def\csname Data/\DataPrefix/height\endcsname{\pgfmathprintnumber{32}}


==> data1/fd/global/basic/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/\DataPrefix/lambda\endcsname{\pgfmathprintnumber{0.02}}
\expandafter\def\csname Data/\DataPrefix/beta\endcsname{\pgfmathprintnumber{0.001}}
\expandafter\def\csname Data/\DataPrefix/tau\endcsname{\pgfmathprintnumber{2000.0}}
\expandafter\def\csname Data/\DataPrefix/maxiters\endcsname{\pgfmathprintnumber{100}}
\expandafter\def\csname Data/\DataPrefix/ninner\endcsname{\pgfmathprintnumber{1000}}
\expandafter\def\csname Data/\DataPrefix/width\endcsname{\pgfmathprintnumber{584}}
\expandafter\def\csname Data/\DataPrefix/height\endcsname{\pgfmathprintnumber{388}}


==> data1/fd/scaling/opticalflow/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/scaling/opticalflow/lambda\endcsname{\ensuremath{0.01}}
\expandafter\def\csname Data/scaling/opticalflow/beta\endcsname{\ensuremath{0.001}}
\expandafter\def\csname Data/scaling/opticalflow/Mdir\endcsname{\ensuremath{6}}
\expandafter\def\csname Data/scaling/opticalflow/ntimings\endcsname{\ensuremath{3}}
\expandafter\def\csname Data/scaling/opticalflow/stopenergy\endcsname{\ensuremath{130.0}}
\expandafter\def\csname Data/scaling/opticalflow/ninner\endcsname{\ensuremath{300}}
\expandafter\def\csname Data/scaling/opticalflow/width\endcsname{\ensuremath{584}}
\expandafter\def\csname Data/scaling/opticalflow/height\endcsname{\ensuremath{388}}


==> data1/fd/surrogate/outerinner/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/\DataPrefix/lambda\endcsname{\pgfmathprintnumber{0.01}}
\expandafter\def\csname Data/\DataPrefix/beta\endcsname{\pgfmathprintnumber{0.001}}
\expandafter\def\csname Data/\DataPrefix/minenergy_maxiters\endcsname{\pgfmathprintnumber{50000}}
\expandafter\def\csname Data/\DataPrefix/maxiters\endcsname{\pgfmathprintnumber{100}}
\expandafter\def\csname Data/\DataPrefix/ninner\endcsname{\pgfmathprintnumber{50}}
\expandafter\def\csname Data/\DataPrefix/M\endcsname{(4, 4)}
\expandafter\def\csname Data/\DataPrefix/overlap\endcsname{(50, 50)}
\expandafter\def\csname Data/\DataPrefix/energymin\endcsname{\pgfmathprintnumber{107.56900190825763}}
\expandafter\def\csname Data/\DataPrefix/width\endcsname{\pgfmathprintnumber{584}}
\expandafter\def\csname Data/\DataPrefix/height\endcsname{\pgfmathprintnumber{388}}


==> data1/fd/surrogate/outerinner_ref/data.tex <==
\providecommand{\Data}[1]{
    \csname Data/#1\endcsname
}
\expandafter\def\csname Data/surrogate/outerinner_ref/lambda\endcsname{\ensuremath{0.002}}
\expandafter\def\csname Data/surrogate/outerinner_ref/beta\endcsname{\ensuremath{0.01}}
\expandafter\def\csname Data/surrogate/outerinner_ref/minenergy_maxiters\endcsname{\ensuremath{10^{6}}}
\expandafter\def\csname Data/surrogate/outerinner_ref/maxiters\endcsname{\ensuremath{10^{2}}}
\expandafter\def\csname Data/surrogate/outerinner_ref/ninner\endcsname{\ensuremath{10^{2}}}
\expandafter\def\csname Data/surrogate/outerinner_ref/M\endcsname{(4, 4)}
\expandafter\def\csname Data/surrogate/outerinner_ref/overlap\endcsname{(5, 5)}
\expandafter\def\csname Data/surrogate/outerinner_ref/width\endcsname{\ensuremath{48}}
\expandafter\def\csname Data/surrogate/outerinner_ref/height\endcsname{\ensuremath{32}}

